Early Scheduling in Parallel State Machine Replication

State machine replication is standard approach to fault tolerance. One of the key assumptions of state machine replication is that replicas must execute operations deterministically and thus serially. To benefit from multi-core servers, some techniques allow concurrent execution of operations in state machine replication. Invariably, these techniques exploit the fact that independent operations (those that do not share any common state or do not update shared state) can execute concurrently. A promising category of solutions trades scheduling freedom for simplicity. This paper generalizes this category of scheduling solutions. In doing so, it proposes an automated mechanism to schedule operations on worker threads at replicas. We integrate our contributions to a popular state machine replication framework and experimentally compare the resulting system to more classic approaches.

==> discussaoConceitual.tex <==
%!TEX root =  main.tex
\clearpage

\section{Internal Discussion}


\subsection{Scheduling Literature}

Handbook of Scheduling. Edited by Joseph Y-T Leung. Chapman and Hall.  2004.   
See our shared dropbox.

https://www.crcpress.com/Handbook-of-Scheduling-Algorithms-Models-and-Performance-Analysis/Leung/p/book/9781584883975

http://www2.informatik.uni-osnabrueck.de/knust/class/


According to the handbook above, it seems we are looking at a: Pm | prec | Cmax  problem.
See the terminology.   Pm stands for parallel, with known number of processor nodes.   prec
is  when jobs have precedence.  Looking at C_max, which is the makespan.

Processors are homogeneous.  Job precedence builds a DAG.   Makespan (see section 1.3 - notation - page 1-8 in the handbook)
is defined as max(C_1, ... C_n), where C_j denotes the completion time of job j.
Since jobs have precedence, the maximum C_j is the completion time of the whole schedule.

These problems typically consider building a schedule for a known set of jobs.

If we take an algorithm like Kotla's, the incoming 'jobs' (= smr requests) are
classified to have or not dependencies w.r.t. other, already delivered, pendent jobs.   
In a given moment, the pendent jobs build a dependency graph.   Taking the pendent jobs, 
Kotla's scheduling algorithm can be seen in page 3-2 of this handbook, under highest-level-first or critical-path or 
Hu's algorithm (1961).   There they discuss jobs with precedence constraints and that this 
algorithm has optimal makespan - as far as i could understand...
The price to build this graph is not an issue in this literature.  It is simply given.

On the other hand, it is part of our problem.
Our approach is based on this aspect: we want to avoid the
price of extracting and building dependencies, or generally, the price to decide how to execute.
Offline scheduling would be when all the scheduling decisions are calculated a priori.
With online scheduling some decision is taken when the job arrives.
Our scheduling is online by nature, but we want to reduce the decision cost.

Considering our execution model, which is quite peculiar, i did not find more direct works to compare.

To show that our scheduling decisions are good, we would have to show that 
for any given (delivered pendent) sequence of commands (jobs), the dependencies 
represented (or induced in the execution) in our model approximate (or only closely extrapolate) 
the needed ones (by Hu's or Kotla's algorithm).

However, to show this starting from the thread to class mapping, class conflicts, class types and so on...
ant then relate/compare to the dependency graph ... seems to be a long path.

But, maybe we can argue in an intuitive level. 
We want to avoid dependency - which is to promote concurrency.
Is it possible to find a concurrency measure for our mappings ?
We could then just maximize concurrency...














==> experimentsSRDS.tex <==
%!TEX root =  main.tex
\clearpage
\section{Experimental evaluation}
\label{exp}
 
In order to assess the performance of parallel state machine replication, we implemented the proposed protocols in the \textsc{Bft-SMaRt} environment~\cite{Bes14} and conducted experiments in Emulab \cite{Whi02}. 
\textsc{Bft-SMaRt} was developed in Java and its atomic broadcast protocol executes a sequence of consensus instances, where each instance orders a batch of requests.
%), but uses a staged message flow with parallelism. Consequently, the resulting system provides sequential 
%atomic broadcasts and parallel operation executions.

\noindent\textbf{Experimental Setup:} The Emulab environment was configured with 5 d710 machines (2.4 GHz 64-bit Intel Quad Core Xeon E5530 with 2 CPU threads per core, 12GB of RAM and 1 Gbps network cards) 
and a 1Gbps switched network. The software installed on the machines was Ubuntu 14 64-bit and a 64-bit Java virtual machine version 1.8.0\_121. For all experiments, 
\textsc{Bft-SMaRt} was configured with three replicas hosted in separate machines to tolerate up to one replica crash, while 90 clients were distributed uniformly across another two machines. 
We evaluated the raw throughput of the system at the servers and the latency perceived at the clients over the course of $300$ seconds.

\noindent\textbf{Goals:}
Our main goal is to analyze the differences among the previously discussed approaches and show how reconfigurations could increase the performance. 
The first set of experiments shows the expressiveness of the classes of requests proposed to model concurrency (Section~\ref{ex:groups}). 
The second set of experiments depicts the behavior of the system under different 
replica configurations (Section~\ref{ex:repl_conf}). Finally, the last 
set of experiments shows how reconfigurations could improve performance (Section~\ref{ex:rec}).

\noindent\textbf{Notation:} 
We use the notation $\texttt{xPyS}$ to represent the configuration with $\texttt{x}$ parallel and $\texttt{y}$ sequential replicas. 
Except for the execution with reconfiguration, parallel replicas were configured with $10$ working threads.

%\subsection{Results and Analysis}


\subsection{Modeling concurrency with classes of requests} 
\label{ex:groups}

To show how concurrency modeling impacts performance, we implemented a tuple space and analyzed the two models defined in Section~\ref{sec:conc_samples}
using the thread mappings ($CtoT$) presented at Section~\ref{sec:parallelism}. 
The tuple space was initialized with $100k$ tuples, with the number of fields uniformly distributed from $1$ to $10$ at each replica.
As for the workload, each client submits one of the possible requests at a time, $rdp$, $inp$, $out$ and $cas$, and all request types appear in equal proportion in the workload. 
The number of fields for a tuple or template in each operation was uniformly distributed from $1$ to $10$.



Figure~\ref{performance_ts} presents the results for sequential and parallel executions for both concurrency models. 
The Simple Tuple Space (TS) concurrency model allows reduced concurrency, resulting in a workload with $75\%$ of conflicting requests.
This significantly impacts performance, which is worse than in a sequential execution ($\texttt{0P3S}$) due to the need for additional synchronization.

  \begin{figure}[!ht]
 \begin{center}
  \subfigure[Throughput]{\label{t-ts}
   \includegraphics[scale=0.45]{new_experiments/tuple_space/th_ts.pdf}}
  \subfigure[Latency]{\label{l-ts}
   \includegraphics[scale=0.45]{new_experiments/tuple_space/latency_ts.pdf}}
  
 \end{center}
 \caption{Sequential vs. parallel executions for two concurrency models.}
 \label{performance_ts}
\end{figure}
 

 The Extended Tuple Space (TS) concurrency model, however, results in performance that is more than twice the performance of the sequential execution. 
In this model, $out$, $rdp$ and $inp$ requests handling tuples or templates with the same number of fields are mapped and sequentially executed by a single thread, but are executed concurrently with other requests for tuples or templates with different number of fields. 
$cas$ requests may be mapped to one or two threads, depending on the request parameters. 
This model improves performance since it only needs to synchronize groups of two threads in $cas$ executions.
No other expensive synchronization among threads is necessary.
These results show that classes of requests can precisely capture the concurrency of an application.

 
\subsection{Replicas with different degrees of parallelism}
\label{ex:repl_conf}

We use a linked list implementation, the concurrency model defined at Section~\ref{sec:conc_samples}, and the thread mapping ($CtoT$) presented at Section~\ref{sec:parallelism} to analyze the performance of deployments in which replicas are statically configured with different degrees of parallelism.
The list was initialized with $100k$ entries at each replica and we used $add$ and $contains$ to represent operations of classes $c_w$ and $c_r$, respectively. 
The parameter for these operations was always the last element in the list.
Consequently, operations in an execution have similar cost, leading to more stable measurements.


Figure~\ref{performance_dc} presents the results for different replica configurations under workloads composed of $contains$ requests only, $add$ requests only, and mixed requests, where clients cycle through $60$-second periods during which one request type is submitted only, starting with $contains$. 
Recall that while $contains$ requests do not conflict with each other, any two $add$ requests conflict.
The throughput presented is the average obtained throughout the execution. 
For workloads with only $contains$ or $add$ requests, there was little variation in throughput and latency during the execution, while for the mixed workload throughput and latency fluctuate over time (more details about the mixed workload in the next section). 
For the mixed workload, we also show the results for the reconfiguration technique (REC).



\begin{figure}[!ht]
  \begin{center}
  \subfigure[Throughput]{
  \includegraphics[scale=0.45]{new_experiments/th/th_dc.pdf}}
  \subfigure[Latency]{
  \includegraphics[scale=0.45]{new_experiments/latency/latency.pdf}}
  \end{center}
  \caption{Different replica configurations.}
  \label{performance_dc}
\end{figure}


\begin{figure*}[ht]
  \begin{center}
  \includegraphics[width=1.4\columnwidth]{new_experiments/output_mix.pdf}
  \end{center}
  \caption{Parallel vs. sequential replica throughput for the mixed workload.}
  \label{tp_dc_mix}
\end{figure*}
 
 \begin{figure*}[!ht]
  \begin{center}
  \subfigure[Sequential vs. Parallel]{
  \includegraphics[width=1.4\columnwidth]{new_experiments/output_mix_seq_pl.pdf}}
  \subfigure[Sequential vs. Reconfigurable]{  
  \includegraphics[width=1.4\columnwidth]{new_experiments/output_mix_seq_rec.pdf}}
  \end{center}
  \caption{Throughput for the mixed workload and reconfigurations.}
  \label{tp_rec_mix}
\end{figure*}


The system with different replica configurations ($\texttt{1P2S}$ and $\texttt{2P1S}$) presented 
better performance for both $contains$ or $add$ workloads, while parallel ($\texttt{3P0S}$) and sequential ($\texttt{0P3S}$) configurations outperform each other in the presence of non-conflicting and conflicting requests, respectively. 
This means that, unlike a traditional P-SMR~\cite{Par14,Par14Opt}, hybrid approaches that mix replicas with different degrees of parallelism provide good performance for both workloads. 
Unfortunately, however, the hybrid approach has two serious drawbacks: \textit{(i)} the resources of the replicas that lag behind could exhaust rapidly, making the replicas crash or drop requests; 
and \textit{(ii)}~it does not provide the best performance for mixed workloads. % that may change over time. 

Figure~\ref{tp_dc_mix} depicts the behavior of a parallel and a sequential replica of configuration $\texttt{1P2S}$ for the mixed workload. 
The figure shows the sequential replica became substantially delayed while executing $contains$ requests and only executed the first $add$ request at time $250$ while the parallel replica executed the first $add$ request at time $60$ seconds.
From second $60$ to $250$, the sequential replica stored approximately $650k$ operations in its buffer, the number of operations executed by the parallel replica in this period.
For workloads with enough non-conflicting requests, this situation would eventually lead to a buffer overflow. 
Ironically, due to the delay, the sequential replica does not help improve performance when requests conflict and the system will run at the pace of the parallel replica, even though the parallel replica is not the best choice for conflicting requests.
We conclude that one cannot optimize performance of state machine replication by mixing replicas with different degrees of parallelism.
 
\subsection{Reconfiguration in action}
\label{ex:rec}

We used the same linked list implementation, configurations and the mixed workload of the previous experiments 
to show how reconfiguration can boost performance. 
Figure~\ref{tp_rec_mix} presents the throughput for sequential ($\texttt{0P3S}$), parallel ($\texttt{3P0S}$) and reconfigurable ($\texttt{REC}$) executions. 
The hybrid systems ($\texttt{1P2S}$ and $\texttt{2P1S}$) presented a behavior similar to the parallel execution since the performance was determinated by parallel 
replicas (see previous discussion about Figure~\ref{tp_dc_mix}).
In the reconfigurable execution, the system started with only $1$ active thread and used the policy of Algorithm~\ref{alg_policy} to activate/deactivate threads, ranging from $1$ to $10$ active threads. 
Figure~\ref{performance_dc} (mixed columns) shows the average throughput and latency perceived by clients.

Reconfiguration improves system performance and, at the same time, saves resources since threads are deactivated when they are unnecessary and their presence may negatively impact performance. 
For example, at time $60$ seconds when clients start to invoke only dependent requests, performance drops to approximately $0.8$ Kops/sec and the system starts to deactivate threads. 
After approximately $10$ seconds, it remains with only one active thread and the throughput becomes similar to a sequential execution (approximately $1.8$ Kops/sec). 
Notice that the policy will define the time to react after a workload change.






==> lessons_arxiv.tex <==
%!TEX root =  main.tex

\subsection{Lessons learned - COMENTADA}
 
 This section presents a few observations about the experimental evaluation.
 
\begin{enumerate}
\item \emph{Early scheduling outperforms late scheduling.}
Despite the fact that early scheduling is more restrictive than late scheduling, it delivers superior performance in almost all cases we considered.
This happens for two reasons:
(1) the early scheduler can make simple and fast decisions, and 
(2) by using one data structure per worker thread, worker threads do not content of a single data structure, as with late scheduling.

 

COMENTARIO dotti - escrevi o que segue, que acho que relaciona com o acima: \\
Fast vs. accurate runtime decisions:
 
As we could notice, in high throughput systems there is  room to discuss 
the tradeoff of fast versus accurate runtime decisions.   Although CBASE does not hinder
the concurrency level (since the dependencies followed are the needed and sufficient ones 
given by service semantics), better throughput results can be achieved with a 
solution trading concurrency for fast runtime decision.   The main reason for this is related
to contention due to the graph structure but it is also relevant to observe that 
since the number of threads (cores) for an application is typically bounded in concrete
implementations, adopting strategies that limit the achievable concurrency level
may still not hinder the concurrency level in concrete settings.

FIM COMENTARIO dotti

\item \emph{The number of workers matters for performance, but not equally for the two scheduling techniques.}
For both schedulers, the ideal number of worker threads depends on the application and workload.
However, the performance impact caused by the number of workers is lower in the late than in the early scheduler.
%:
%except for the write-only workload, most experiments presented a better performance with 12 workers. 
This observation suggests that both scheduling techniques can benefit from a reconfiguration protocol~\cite{Alchieri2017} to adapt the number of workers on-the-fly.

%\item In the early scheduler, the number of threads working for a requests class can be configured according to the workload by using weights. 
% In case of a workload change, this number can be adapted at runtime~\cite{Alchieri2017}. 
 
\item \emph{Choosing the right data structures is fundamental to performance.}
Since all requests must go through the same data structure, the performance of late scheduler is bounded by requests with worst performance.
The early scheduler uses a queue per worker and does not force workers to synchronize in the presence of independent requests.
Moreover, requests of one class do not impact performance of requests in other classes.
 

COMENTARIO dotti: \\
NAO SEI SE CONCORDO COM A PRIMEIRA FRASE ACIMA: requests independentes podem ser processados concorrentemente em ambas tecnicas.
acho que perdi alguma sutileza ... talvez uma clarificacao.
Parece-me que esta observacao estaria contida na 1 acima.  
Nao sei se devemos bater mais no fato do CBASE ser uma secao critica unica.   tivemos uma critica nisso...

FIM COMENTARIO dotti

COMENTARIO dotti: sugestao para a questao do naive \\

\item \emph{Class to thread assignment needs information about all classes.}
A local view of related classes was not sufficient to reach good (in terms of the optimization objective) assignments.
The naive thread assignment shows this.  While it may seem acceptable to configure concurrent classes
distributing threads proportionally to their demands and then assure that sequential classes synchronize with
the other classes as needed, it has been observed that analysing the whole conflict relation 
could be worthy to consider a class as sequential (even it could be concurrent) to avoid further 
inducing synchronization with other classes.  
Whether this assignment problem can be partitioned (according to the class conflict topology) 
is still to be analysed.

FIM COMENTARIO dotti

\end{enumerate}










==> optimizer-dotti.tex <==
%!TEX root =  main.tex
\section{Optimized scheduling in parallel \\ state machine replication}
\label{sec:optm}
\label{sec:optimization}

In this section, we formulate the problem of mapping a request classes definition to a set of worker threads.
The mapping assumes the execution model described in the previous section.

\subsection{The optimization model}

The mapping of threads to classes is shaped as an optimization problem that starting with some input data  must produce an output that satisfies a number of constraints and optimizes a condition (see Algorithm~\ref{model}).

\subsubsection{Input and output}

The inputs are the request classes definition and a set of threads available with their relative weight information.
\begin{itemize}
\item the classes $C = \{c_1, .., c_{nc} \}$, as in Def. \ref{def.rClasses};
\item $\# = C \times C$, the class conflict relation derived from $\mathcal{R}$ in Def. \ref{def.rClasses} 
where $(c_1,c_2) \in \# $ iff $ (c_1 \rightarrow (c_{set},r_{set})) \in \mathcal{R} \ and \ c_2 \in c_{set} $;
\item $T = \{ t_1, .., t_{nt} \}$, the set of threads to map classes;
\item $W = C \times  \mathbb{R}$, the relative weight classes.  The weight is used to represent the computational work imposed by each class being relative among threads and used distribute  threads to classes.
\end{itemize}


The optimization of this model has as outputs the mapping from classes to threads and the choice of which 
classes are considered internally conflicting according to discussed in IR.3 above.
The output is the classes to threads mapping as well as the definition of which classes are sequential.
These are variables $uses$ and $Seq$ in Algorithm~\ref{model}.
This is the complete information for the scheduler: when a request $r$ belonging to a class $c$ arrives,
the scheduler dispatches $r$ to all or any one of the threads used by $c$ ($uses{C,T}$) if the class 
is respectively $Sec$ or $Cnc$ ($Cnc = \lnot Seq$).

\subsubsection{Constraints} 
%{\bf We then argue that the execution of this scheduling respects $\prec_R$ ?}.  

The set of restrictions to the mapping should ensure that implementation rules IR.0, IR.3, IR.4 and IR.5 are followed,
while IR.1 and IR.2 are ensured by the scheduler implementation, which ensures that the execution is correct w.r.t. ordering
as already discussed.

\subsubsection{Objective function} 

The restrictions imposed by the implementation rules may be satisfied by several associations of threads to classes. 
Among those, to maximize the global throughput, we are interested in the ones where:
\begin{itemize}
\item O.1: internally concurrent classes use several threads to favor throughput;
\item O.2: sequential classes should use only the needed threads for classes synchronization and avoid extra thread usage
since synchronization penalizes performance; 
\item O.2: thread distribution across classes consider the weight of the classes;
\item O.3: non conflicting classes with internal conflict use separate subsets of threads to avoid synchronization.
\end{itemize}

%The above discussed optimization model was implemented with AMPL \cite{AMPL} modeling language.


\begin{algorithm}[ht!]
\floatname{OptModel}{Model}
\caption{Optimization model.}
\footnotesize{
\begin{distribalgo}[1]
\label{model} 

\INDENT{\textbf{input:}}
%	\REQUIRE  \COMMENT{classes, conflicts and threads} \\
	\vspace{1mm}
	\STATE $set \ C$ \label{lC} 
	\COMMENT{\hfill // set of request classes}
	\vspace{1mm}
	\STATE $set \ T$ \label{lT}
	\COMMENT{\hfill // set of threads}
	\vspace{1mm}
	\STATE $w\{C\} \in \mathcal{R}$ \label{lw}
	\COMMENT{\hfill // relative weight of each class}
	\vspace{1mm}
	\STATE $\#\{C_i,C_j\} \in \{ 0, 1 \}$ \label{lconflicts}
	\COMMENT{\hfill // $\#[c_i,c_j] = 1$\ :\ $c_i$ and $c_j$ conflict}
	\vspace{1mm}
%	\STATE $wc = \sum_{\forall c \in C\ :\ Cnc[c]} w[c]$
%	\COMMENT{\hfill // weights of concurrent classes}
%	\vspace{1mm}
\ENDINDENT

\INDENT{\textbf{output:}}
%	\REQUIRE \COMMENT{the mapping and internal conflict as in R2 } \\
	\vspace{1mm}
	\STATE $uses\{C,T\} \in \{ 0, 1 \}$ \label{luses} 
	\COMMENT{\hfill // uses[c,t] = 1 : class $c$ uses thread $t$}   
	\vspace{1mm}
	\STATE $Seq\{C\} \in \{ 0, 1 \}$ \label{ldep}
	\COMMENT{\hfill  // $Seq(c) = 1$ : $c$ is sequential}
	\vspace{1mm}
%	\STATE $Cnc\{C\} = \lnot Seq\{C\} \in \{ 0, 1 \}$ \label{ldep2}
%	\COMMENT{\hfill  // $Cnc(c) = 1$ : $c$ is concurrent}
%	\vspace{1mm}
\ENDINDENT

\INDENT{\textbf{auxiliary definitions:}}
	\vspace{1mm}
	\STATE $nc = |C|$
	\COMMENT{\hfill  // number of classes}
	
	\vspace{1mm}
	\STATE $nt = |T|$
	\COMMENT{\hfill  // number of worker threads}
	
	\vspace{1mm}
	\STATE $Cnc\{C\} = \lnot Seq\{C\} \in \{ 0, 1 \}$ \label{ldep2}
	\COMMENT{\hfill  // $Cnc(c) = 1$ : $c$ is concurrent}

	\vspace{1mm}
	\STATE $wc = \sum_{\forall c \in C\ :\ Cnc[c]} w[c]$
	\COMMENT{\hfill // weights of concurrent classes}

	\vspace{1mm}
\ENDINDENT


\INDENT{\textbf{constraints:}}
	\vspace{1mm}
	\STATE $\forall c \in C \ :\  \bigvee_{\forall t \in T} uses(c,t)$ \label{lIR0}
	\COMMENT{\hfill // R.0}
	\vspace{2mm}
	
	\STATE $\forall c \in C \ :\  \#[c_1,c_1] \Rightarrow Seq[c_1]$ \label{lIR1}
	\COMMENT{\hfill // R.1}
	\vspace{2mm}
	
	\STATE $\forall c_1, c_2 \in C \ :\ \#[c_1,c_2] \Rightarrow Seq[c_1] \lor Seq[c_2]$ \label{lIR3}
	\COMMENT{\hfill // R.3}
	\vspace{2mm}

	\STATE $\forall c_1, c_2 \in C, t \in T \ :\ $ \\
		\hfill $\#[c_1,c_2] \land Seq[c_1] \land Cnc[c_2] \land uses[c_2,t] \Rightarrow uses[c_1,t]$ \label{lIR4}
 	\COMMENT{\hfill // R.4}
	\vspace{2mm}

	\STATE $\forall c_1, c_2 \in C \ :\ \#[c_1,c_2] \land Seq[c_1] \land Seq[c_2] \Rightarrow $ \\
		\hfill $\exists t \in T \ :\ uses[c_1,t] \land uses[c_2,t]$ \label{lIR5}
	\COMMENT{\hfill // R.5}
	\vspace{1mm}
\ENDINDENT

 
\INDENT{\textbf{objective:}}
	\vspace{1mm}
	\STATE minimize cost:
	\vspace{2mm}

	\STATE $ - \sum_{\forall c \in C \,:\, Cnc[c]} |\{t \in T \,:\, uses[c,t]\}|$ \label{lobjinit}
	\COMMENT{\hfill // O.1}
	\vspace{2mm}

    \sum_{\forall c \in C \,:\, Cnc[c] \times \sum{t \in T} 
    sum {c in C} ( (1-dep[c]) * (sum{t in T}uses[c,t]*w[c]) ) 
            /
            ( sum{c2 in C}( (1-dep[c2])*w[c2] ) )


	\STATE $ + \sum_{\forall c \in C \,:\, Cnc[c]} w[c]/wc -$ \\
		\hfill $(|\{\forall t \in T:uses[c,t]\}|/ \mathit{nt} ) | \times \mathit{nt}$ \label{lobjloadb} 
	\COMMENT{\hfill // O.2}
	\vspace{2mm}

	\STATE $ + \sum_{\forall c_1, c_2 \in C \ s.t. \ Seq[c_1] \land Seq[c_2] \land \lnot \#[c_1,c_2]}$ \\
		\hfill $card(\{\forall t \in T \ s.t. \ uses[c_1,t] \land uses[c_2,t] \} )$ $\times 2 \times nt \times nc$ \label{lobjend} \label{lobj2ndpart}
	\COMMENT{\hfill // O.3}
	\vspace{2mm}
\ENDINDENT
      
\end{distribalgo}
}
\end{algorithm}

In lines \ref{lC} to \ref{lconflicts} we have the inputs to the problem, with the set of classes, their conflict relation, their relative weight and the set of threads to be mapped to.
As output we have the information if a given thread is used by a class, in line \ref{luses} and if the class is considered as internally sequential or concurrent for execution, see lines \ref{ldep} and \ref{ldep2}.
The restrictions discussed before are presented in lines \ref{lIR0} to \ref{lIR5}.  
In line \ref{lIR0} it is stated that for each class, at least one thread is associated.
In line \ref{lIR3} it is stated that if any two classes conflict then at least one of them is sequential.
In line \ref{lIR4} it is stated that if any two classes conflict, one of them is internally concurrent and the other sequential,
then all threads associated to the concurrent class are also in the sequential.
In line \ref{lIR5} it is stated that if any two classes conflict and both are sequential,
then there exists at least one common thread in both classes.

The objective function to minimize is presented in lines \ref{lobjinit} to \ref{lobjend}.
Beginning in \ref{lobjinit}, O.1, we have
a reward to the use of threads by internally concurrent classes, improving concurrency.
%
In O.2. we have that the use of threads by concurrent classes is proportional to their weight.  More concretely, we minimize the difference of the normalized weight of each class to its proportional use of available threads.  
We multiply this term by the number of threads in the system to make it compatible with the previous term.
%
The third part of the optimization function, O.3, applies a penalty to solutions that introduce common threads to non conflicting classes that have internal conflict.  The reason is that this would impose unneeded synchronization and thus impact throughput.
In line \ref{lobjend} we multiply this term such that it gains in priority with regard to the others.

%\subsection{Solving the optimization problem}
The optimization problem was described with the AMPL language \cite{fourer1993ampl} and solved with the KNitro solver \cite{Byrd06knitro:an}.

\subsection{Example}

Let us consider the generalized sharded service with single- and multi-shard read and write requests.
We take the example with 2 partitions, 8 threads, where all classes have same weight.  The input 
parameters are: set $C=\{C_{R1}, C_{W1}, C_{R2}, C_{W2}, C_{Rg}, C_{Wg} \}; set $T = \{1, 2, 3, 4, 5, 6, 7, 8\};
$w$, that associates 1 to all classes; and the conflict topology presented in Fig. \ref{fig:cclasses}(c) 
which is input in the $conflicts\{C,C\}$ parameter.

According to the optimization model, we have the following output to variable $Seq$:

 \begin{figure}[!ht]
  \begin{center}
  \includegraphics[width=0.9\columnwidth]{figs/classthreads1.pdf}
  \includegraphics[width=0.9\columnwidth]{figs/classthreads1.pdf}
  \end{center}
  \caption{Bla bla bla}
  \label{fig:classthreads}
\end{figure}



%%\begin{table}
%\begin{center}
%\begin{footnotesize}
%\begin{tabular}{|c|c|c|c|c|c|c|c|}
%\hline
%class    & $C_{Rg}$ & $C_{Wg}$ & $C_{R1}$  & $C_{R2}$ & $C_{W1}$ & $C_{W2}$  \\ 
%\hline
%Seq & T & T & F & F & T & T   \\ 
%\hline
%\end{tabular}
%\end{footnotesize}
%\end{center}
%% \caption{Output var $Sec\{C\}$}
%%\end{table} 
%
%The following thread association to each class in $uses$:
%
%\begin{center}
%\begin{footnotesize}
%\begin{tabular}{|c|c|c|c|c|c|c|c|}
%\hline
%& $C_{Rg}$ & $C_{Wg}$ & $C_{R1}$  & $C_{R2}$ & $C_{W1}$ & $C_{W2}$   \\ 
%\hline
%1 &  0 &  1 &  1  & 0  & 1 &  0  \\ \hline
%2 &  0 &  1 &  1  & 0  & 1 &  0 \\ \hline
%3 &  0 &  1 &  1  & 0  & 1 &  0 \\ \hline
%4 &  0 &  1 &  0  & 1  & 0 &  1 \\ \hline
%5 &  1 &  1 &  0  & 1  & 0 &  1 \\ \hline
%6 &  0 &  1 &  1  & 0  & 1 &  0 \\ \hline
%7 &  1 &  1 &  1  & 0  & 1 &  0 \\ \hline
%8 &  0 &  1 &  0  & 1  & 0 &  1 \\ \hline
%
%\end{tabular}
%\end{footnotesize}
%\end{center}
%% \caption{Output var $uses\{C,C\}$}
 
 
We notice that reads and writes in shards 1 and 2 use disjoint sets of threads, and that threads are distributed evenly among these classes.   Since reads in one shard can be concurrent but conflict with writes, the write class has all threads associated to the respective read class.   Global writes have to have a fixed order relative to all other operations, therefore all threads synchronize to execute a global write.    A global read is concurrent by the input conflict definition. Since $C_{Rg}$ conflicts with $C_{W1}$ and $C_{W2}$, to keep $C_{Rg}$ concurrent all threads that implement $C_{Rg}$ would have to be included in  $C_{W1}$ and $C_{W2}$.   Doing so, $C_{W1}$ and $C_{W2}$ would not be disjoint and thus synchronize even if no global read request is being processed.   A cheaper solution is to define $C_{Rg}$ as $Seq$ and associate to it one thread of each of the shards.  This means that whenever a global read takes place, it synchronizes its threads to execute in the shards.  Since writes in the shards are sequential, the global read will take place in a well defined order.
 
 


%
%
% while $c_2$ has no internal conflict, then the set of threads associated to $c_2$ must be included in the set of threads associated to $c1$.   This ensures that any request processed by $c_2$ has an order relative to $c_1$ because $c_1$ synchronize all its threads (which include those of $c_2$) to execute its requests. 
%
%\item R2: a thread may be associated to any number of classes, from 0 to $nc$; 
%\item R3: a class without internal conflict $c_c$ ($c$oncurrent) schedules a request to any one of its threads;
%\item R4: a class with internal conflict $c_d$ ($d$ependent) schedules a request to all of its threads (see execution model);
%
%\item R5: different, conflicting classes have to have overlapping sets of threads;
%\item R5.1: if two internally conflicting classes conflict, then they need at least one common thread to assure total order among them (see R4);
%\item R5.2: if one internally conflicting class $c_d$ conflicts with one internally non-conflicting class $c_c$, it suffices that threads of $c_c$ are contained in threads of $c_d$.  Since $c_d$ schedules the requests to all its threads, the synchronous execution of a request in all of $c_c$ threads creates a  total order among classes, although $c_c$ requests are concurrent among them;
%\item R5.3: if two internally non conflicting classes conflict (even this case may be rare), the total order among classes has to be respected.   It suffices to reduce this case to R5.2 by assuming as if one of the classes would be internally conflicting and thus granting the same as R5.2.
%\end{itemize}
%
%The choice of which classes should be considered internally conflicting (discussed R5.3) should minimize the number of 
%internally conflicting classes in the system, since they reduce concurrency. This choice depends only on the topology of dependencies among classes and is irrespective of the mapping to threads.  
%We solve this problem in a separate optimization problem, before mapping threads to classes, defined as follows.

%Given inputs:
%\begin{itemize}
%\item the classes $C = \{c_1, .., c_{nc} \}$;
%\item $ClassConflict = C \times C$, the class conflict relation;
%\end{itemize}
%
%Calculate the output:
%\begin{itemize}
%\item $ClassType = C \times  \{ conc, dep\}$, where $conc$ means internally concurrent and $dep$ means internally dependent;
%\end{itemize}
%
%With the following restrictions:
%\begin{itemize}
%\item if a class conflicts internally, it is of type $dep$, i.e.:  $\forall (c,c) \in ClassConflict, (c,dep) \in ClassType$;
%\item if two classes conflict, at least one is $dep$, i.e.: $\forall (c_a, c_b) \in ClassConflict, ((c_a,dep) \in ClassType) \vee (c_b,dep) \in ClassType))$;
%\item all other classes are $conc$.
%\end{itemize}
%
%Subject to minimizing the number of $dep$ classes, i.e.: 
%$$ minimize ~ \sum_{\forall c \in C} (c,dep) \in ClassType$$
%
%Having fixed the types of classes as above, we now have to solve a second optimization problem with restrictions R1 to R5.2 above to, having as inputs:
%\begin{itemize}
%\item the classes $C = \{c_1, .., c_{nc} \}$;
%\item $ClassConflict = C \times C$, the class conflict relation;
%\item $ClassType = C \times  \{ conc, dep\}$, where $conc$ means internally concurrent and $dep$ means internally dependent;
%\item $T = \{ t_1, .., t_{nt} \}$, the set of threads to map classes.
%\end{itemize}
%
%Our output should be 
%\begin{itemize}
%\item $CtoT = C \rightarrow \mathcal{P}(T)$.
%\end{itemize}
%
%To formulate the objective function for this second optimization step we adapt the concept of makespan \cite{????}  to our problem.
%\begin{itemize}
%\item Each thread of the system will be associated to $0$ to $nc$ classes.
%\item We compute the amount of work of each of the $nt$ threads when one unit of work for each
%of the $nc$ classes is submitted to the system.   We call the makespan of threat $t$ caused
%by class $c$, $ms_{(t,c)}$. The total makespan of threat $t$ due to all classes we call $ms_t$.  
%\item If a class $c_a$ is $conc$, associated to a subset of threads $T_a$, the
%the amount of work of each thread of this subset to accomplish a unit of work from $c_a$
%is assumed $1/card(T_a)$, which is $ms_{(i,c_a)}$.  $ms_{(i,c_a)}$ is added to $ms_i$ for all threads $i$ in $T_a$.
%\item If a class $c_b$ is internally conflicting, associated to a subset of threads $T_b$, the amount
%of work of each thread of this subset to accomplish a unit of work from $c_b$, $ms_{(j,c_b)}$, is assumed $1$,
%which is added to $ms_j$ for all threads $j$ in $T_b$.
%\item The objective function is to minimize the maximum makespan among all threads in the system.  
%\begin{itemize}
%\item This leads to a fair load distribution since minimizing the maximum will flatten the makespan value
%distribution across threads.  
%\item To minimize the maximum makespan also leads to minimizing the number of 
%overlapps among thread sets of different classes.  
%\item For independent classes, this leads to maximum thread usage, favoring concurrency.
%\end{itemize}


==> optimizer__Fernando_Dotti_s_conflicted_copy_2017-11-30_.tex <==
%!TEX root =  main.tex
\section{Optimized scheduling in parallel \\ state machine replication}
\label{sec:optm}
\label{sec:optimization}

In this section, we formulate the problem of mapping a request classes definition to a set of worker threads.
The mapping assumes the execution model described in the previous section.

\subsection{The optimization model}

The mapping of threads to classes is shaped as an optimization problem that starting with some input data  must produce an output that satisfies a number of constraints and optimizes a condition (see Algorithm~\ref{model}).

\subsubsection{Input and output}

The inputs are the request classes definition and a set of threads available with their relative weight information.
\begin{itemize}
\item the classes $C = \{c_1, .., c_{nc} \}$, as in Def. \ref{def.rClasses};
\item $\# = C \times C$, the class conflict relation derived from $\mathcal{R}$ in Def. \ref{def.rClasses} 
where $(c_1,c_2) \in \# $ iff $ (c_1 \rightarrow (c_{set},r_{set})) \in \mathcal{R} \ and \ c_2 \in c_{set} $;
\item $T = \{ t_1, .., t_{nt} \}$, the set of threads to map classes;
\item $W = C \times  \mathbb{R}$, the relative weight classes.  The weight is used to represent the computational work imposed by each class being relative among threads and used distribute  threads to classes.
\end{itemize}


The optimization of this model has as outputs the mapping from classes to threads and the choice of which 
classes are considered internally conflicting according to discussed in IR.3 above.
The output is the classes to threads mapping as well as the definition of which classes are sequential.
These are variables $uses$ and $Seq$ in Algorithm~\ref{model}.
This is the complete information for the scheduler: when a request $r$ belonging to a class $c$ arrives,
the scheduler dispatches $r$ to all or any one of the threads used by $c$ ($uses{C,T}$) if the class 
is respectively $Sec$ or $Cnc$ ($Cnc = \lnot Seq$).

\subsection{Constraints} 
%{\bf We then argue that the execution of this scheduling respects $\prec_R$ ?}.  

The set of restrictions to the mapping should ensure that implementation rules IR.0, IR.3, IR.4 and IR.5 are followed,
while IR.1 and IR.2 are ensured by the scheduler implementation, which ensures that the execution is correct w.r.t. ordering
as already discussed.

\subsection{Objective function} 

The restrictions imposed by the implementation rules may be satisfied by several associations of threads to classes. 
Among those, to maximize the global throughput, we are interested in the ones where:
\begin{itemize}
\item O.1: internally concurrent classes use several threads to favor throughput;
\item O.2: sequential classes should use only the needed threads for classes synchronization and avoid extra thread usage
since synchronization penalizes performance; 
\item O.2: thread distribution across classes consider the weight of the classes;
\item O.3: non conflicting classes with internal conflict use separate subsets of threads to avoid synchronization.
\end{itemize}

%The above discussed optimization model was implemented with AMPL \cite{AMPL} modeling language.


\begin{algorithm}[ht!]
\floatname{OptModel}{Model}
\caption{Optimization model.}
\footnotesize{
\begin{distribalgo}[1]
\label{model} 

\INDENT{\textbf{input:}}
%	\REQUIRE  \COMMENT{classes, conflicts and threads} \\
	\vspace{1mm}
	\STATE $set \ C$ \label{lC} 
	\COMMENT{\hfill // set of request classes}
	\vspace{1mm}
	\STATE $set \ T$ \label{lT}
	\COMMENT{\hfill // set of threads}
	\vspace{1mm}
	\STATE $w\{C\} \in \mathcal{R}$ \label{lw}
	\COMMENT{\hfill // relative weight of each class}
	\vspace{1mm}
	\STATE $\#\{C_i,C_j\} \in \{ 0, 1 \}$ \label{lconflicts}
	\COMMENT{\hfill // $\#[c_i,c_j] = 1$\ :\ $c_i$ and $c_j$ conflict}
	\vspace{1mm}
%	\STATE $wc = \sum_{\forall c \in C\ :\ Cnc[c]} w[c]$
%	\COMMENT{\hfill // weights of concurrent classes}
%	\vspace{1mm}
\ENDINDENT

\INDENT{\textbf{output:}}
%	\REQUIRE \COMMENT{the mapping and internal conflict as in R2 } \\
	\vspace{1mm}
	\STATE $uses\{C,T\} \in \{ 0, 1 \}$ \label{luses} 
	\COMMENT{\hfill // uses[c,t] = 1 : class $c$ uses thread $t$}   
	\vspace{1mm}
	\STATE $Seq\{C\} \in \{ 0, 1 \}$ \label{ldep}
	\COMMENT{\hfill  // $Seq(c) = 1$ : $c$ is sequential}
	\vspace{1mm}
%	\STATE $Cnc\{C\} = \lnot Seq\{C\} \in \{ 0, 1 \}$ \label{ldep2}
%	\COMMENT{\hfill  // $Cnc(c) = 1$ : $c$ is concurrent}
%	\vspace{1mm}
\ENDINDENT

\INDENT{\textbf{auxiliary definitions:}}
	\vspace{1mm}
	\STATE $nc = |C|$
	\COMMENT{\hfill  // number of classes}
	
	\vspace{1mm}
	\STATE $nt = |T|$
	\COMMENT{\hfill  // number of worker threads}
	
	\vspace{1mm}
	\STATE $Cnc\{C\} = \lnot Seq\{C\} \in \{ 0, 1 \}$ \label{ldep2}
	\COMMENT{\hfill  // $Cnc(c) = 1$ : $c$ is concurrent}

	\vspace{1mm}
	\STATE $wc = \sum_{\forall c \in C\ :\ Cnc[c]} w[c]$
	\COMMENT{\hfill // weights of concurrent classes}

	\vspace{1mm}
\ENDINDENT


\INDENT{\textbf{constraints:}}
	\vspace{1mm}
	\STATE $\forall c \in C \ :\  \bigvee_{\forall t \in T} uses(c,t)$ \label{lIR0}
	\COMMENT{\hfill // R.0}
	\vspace{2mm}
	
	\STATE $\forall c \in C \ :\  \#[c_1,c_1] \Rightarrow Seq[c_1]$ \label{lIR1}
	\COMMENT{\hfill // R.1}
	\vspace{2mm}
	
	\STATE $\forall c_1, c_2 \in C \ :\ \#[c_1,c_2] \Rightarrow Seq[c_1] \lor Seq[c_2]$ \label{lIR3}
	\COMMENT{\hfill // R.3}
	\vspace{2mm}

	\STATE $\forall c_1, c_2 \in C, t \in T \ :\ $ \\
		\hfill $\#[c_1,c_2] \land Seq[c_1] \land Cnc[c_2] \land uses[c_2,t] \Rightarrow uses[c_1,t]$ \label{lIR4}
 	\COMMENT{\hfill // R.4}
	\vspace{2mm}

	\STATE $\forall c_1, c_2 \in C \ :\ \#[c_1,c_2] \land Seq[c_1] \land Seq[c_2] \Rightarrow $ \\
		\hfill $\exists t \in T \ :\ uses[c_1,t] \land uses[c_2,t]$ \label{lIR5}
	\COMMENT{\hfill // R.5}
	\vspace{1mm}
\ENDINDENT

 
\INDENT{\textbf{objective:}}
	\vspace{1mm}
	\STATE minimize cost:
	\vspace{2mm}

	\STATE $ - \sum_{\forall c \in C \,:\, Cnc[c]} |\{t \in T \,:\, uses[c,t]\}|$ \label{lobjinit}
	\COMMENT{\hfill // O.1}
	\vspace{2mm}

	\STATE $ + \sum_{\forall c \in C \,:\, Cnc[c]} w[c]/wc -$ \\
		\hfill $(|\{\forall t \in T:uses[c,t]\}|/ \mathit{nt} ) | \times \mathit{nt}$ \label{lobjloadb} 
	\COMMENT{\hfill // O.2}
	\vspace{2mm}

	\STATE $ + \sum_{\forall c_1, c_2 \in C \ s.t. \ Seq[c_1] \land Seq[c_2] \land \lnot \#[c_1,c_2]}$ \\
		\hfill $card(\{\forall t \in T \ s.t. \ uses[c_1,t] \land uses[c_2,t] \} )$ $\times 2 \times nt \times nc$ \label{lobjend} \label{lobj2ndpart}
	\COMMENT{\hfill // O.3}
	\vspace{2mm}
\ENDINDENT
      
\end{distribalgo}
}
\end{algorithm}

In lines \ref{lC} to \ref{lconflicts} we have the inputs to the problem, with the set of classes, their conflict relation, their relative weight and the set of threads to be mapped to.
As output we have the information if a given thread is used by a class, in line \ref{luses} and if the class is considered as internally sequential or concurrent for execution, see lines \ref{ldep} and \ref{ldep2}.
The restrictions discussed before are presented in lines \ref{lIR0} to \ref{lIR5}.  
In line \ref{lIR0} it is stated that for each class, at least one thread is associated.
In line \ref{lIR3} it is stated that if any two classes conflict then at least one of them is sequential.
In line \ref{lIR4} it is stated that if any two classes conflict, one of them is internally concurrent and the other sequential,
then all threads associated to the concurrent class are also in the sequential.
In line \ref{lIR5} it is stated that if any two classes conflict and both are sequential,
then there exists at least one common thread in both classes.

The objective function to minimize is presented in lines \ref{lobjinit} to \ref{lobjend}.
Beginning in \ref{lobjinit}, O.1, we have
a reward to the use of threads by internally concurrent classes, improving concurrency.
%
In O.2. we have that the use of threads by concurrent classes is proportional to their weight.  More concretely, we minimize the difference of the normalized weight of each class to its proportional use of available threads.  
We multiply this term by the number of threads in the system to make it compatible with the previous term.
%
The third part of the optimization function, O.3, applies a penalty to solutions that introduce common threads to non conflicting classes that have internal conflict.  The reason is that this would impose unneeded synchronization and thus impact throughput.
In line \ref{lobjend} we multiply this term such that it gains in priority with regard to the others.

%\subsection{Solving the optimization problem}
The optimization problem was described with the AMPL language \cite{fourer1993ampl} and solved with the KNitro solver \cite{Byrd06knitro:an}.

\subsection{Example}

Let us consider the generalized sharded service with single- and multi-shard read and write requests.
We take the example with 2 partitions, 8 threads, where all classes have same weight.  The input 
parameters are: set $C=\{C_{R1}, C_{W1}, C_{R2}, C_{W2}, C_{Rg}, C_{Wg} \}; set $T = \{1, 2, 3, 4, 5, 6, 7, 8\};
$w$, that associates 1 to all classes; and the conflict topology presented in Fig. \ref{fig:cclasses}(c) 
which is input in the $conflicts\{C,C\}$ parameter.

According to the optimization model, we have the following output to variable $Seq$:

 \begin{figure}[!ht]
  \begin{center}
  \includegraphics[width=0.9\columnwidth]{figs/classthreads1.pdf}
  \includegraphics[width=0.9\columnwidth]{figs/classthreads1.pdf}
  \end{center}
  \caption{Bla bla bla}
  \label{fig:classthreads}
\end{figure}



%%\begin{table}
%\begin{center}
%\begin{footnotesize}
%\begin{tabular}{|c|c|c|c|c|c|c|c|}
%\hline
%class    & $C_{Rg}$ & $C_{Wg}$ & $C_{R1}$  & $C_{R2}$ & $C_{W1}$ & $C_{W2}$  \\ 
%\hline
%Seq & T & T & F & F & T & T   \\ 
%\hline
%\end{tabular}
%\end{footnotesize}
%\end{center}
%% \caption{Output var $Sec\{C\}$}
%%\end{table} 
%
%The following thread association to each class in $uses$:
%
%\begin{center}
%\begin{footnotesize}
%\begin{tabular}{|c|c|c|c|c|c|c|c|}
%\hline
%& $C_{Rg}$ & $C_{Wg}$ & $C_{R1}$  & $C_{R2}$ & $C_{W1}$ & $C_{W2}$   \\ 
%\hline
%1 &  0 &  1 &  1  & 0  & 1 &  0  \\ \hline
%2 &  0 &  1 &  1  & 0  & 1 &  0 \\ \hline
%3 &  0 &  1 &  1  & 0  & 1 &  0 \\ \hline
%4 &  0 &  1 &  0  & 1  & 0 &  1 \\ \hline
%5 &  1 &  1 &  0  & 1  & 0 &  1 \\ \hline
%6 &  0 &  1 &  1  & 0  & 1 &  0 \\ \hline
%7 &  1 &  1 &  1  & 0  & 1 &  0 \\ \hline
%8 &  0 &  1 &  0  & 1  & 0 &  1 \\ \hline
%
%\end{tabular}
%\end{footnotesize}
%\end{center}
%% \caption{Output var $uses\{C,C\}$}
 
 
We notice that reads and writes in shards 1 and 2 use disjoint sets of threads, and that threads are distributed evenly among these classes.   Since reads in one shard can be concurrent but conflict with writes, the write class has all threads associated to the respective read class.   Global writes have to have a fixed order relative to all other operations, therefore all threads synchronize to execute a global write.    A global read is concurrent by the input conflict definition. Since $C_{Rg}$ conflicts with $C_{W1}$ and $C_{W2}$, to keep $C_{Rg}$ concurrent all threads that implement $C_{Rg}$ would have to be included in  $C_{W1}$ and $C_{W2}$.   Doing so, $C_{W1}$ and $C_{W2}$ would not be disjoint and thus synchronize even if no global read request is being processed.   A cheaper solution is to define $C_{Rg}$ as $Seq$ and associate to it one thread of each of the shards.  This means that whenever a global read takes place, it synchronizes its threads to execute in the shards.  Since writes in the shards are sequential, the global read will take place in a well defined order.
 
 


%
%
% while $c_2$ has no internal conflict, then the set of threads associated to $c_2$ must be included in the set of threads associated to $c1$.   This ensures that any request processed by $c_2$ has an order relative to $c_1$ because $c_1$ synchronize all its threads (which include those of $c_2$) to execute its requests. 
%
%\item R2: a thread may be associated to any number of classes, from 0 to $nc$; 
%\item R3: a class without internal conflict $c_c$ ($c$oncurrent) schedules a request to any one of its threads;
%\item R4: a class with internal conflict $c_d$ ($d$ependent) schedules a request to all of its threads (see execution model);
%
%\item R5: different, conflicting classes have to have overlapping sets of threads;
%\item R5.1: if two internally conflicting classes conflict, then they need at least one common thread to assure total order among them (see R4);
%\item R5.2: if one internally conflicting class $c_d$ conflicts with one internally non-conflicting class $c_c$, it suffices that threads of $c_c$ are contained in threads of $c_d$.  Since $c_d$ schedules the requests to all its threads, the synchronous execution of a request in all of $c_c$ threads creates a  total order among classes, although $c_c$ requests are concurrent among them;
%\item R5.3: if two internally non conflicting classes conflict (even this case may be rare), the total order among classes has to be respected.   It suffices to reduce this case to R5.2 by assuming as if one of the classes would be internally conflicting and thus granting the same as R5.2.
%\end{itemize}
%
%The choice of which classes should be considered internally conflicting (discussed R5.3) should minimize the number of 
%internally conflicting classes in the system, since they reduce concurrency. This choice depends only on the topology of dependencies among classes and is irrespective of the mapping to threads.  
%We solve this problem in a separate optimization problem, before mapping threads to classes, defined as follows.

%Given inputs:
%\begin{itemize}
%\item the classes $C = \{c_1, .., c_{nc} \}$;
%\item $ClassConflict = C \times C$, the class conflict relation;
%\end{itemize}
%
%Calculate the output:
%\begin{itemize}
%\item $ClassType = C \times  \{ conc, dep\}$, where $conc$ means internally concurrent and $dep$ means internally dependent;
%\end{itemize}
%
%With the following restrictions:
%\begin{itemize}
%\item if a class conflicts internally, it is of type $dep$, i.e.:  $\forall (c,c) \in ClassConflict, (c,dep) \in ClassType$;
%\item if two classes conflict, at least one is $dep$, i.e.: $\forall (c_a, c_b) \in ClassConflict, ((c_a,dep) \in ClassType) \vee (c_b,dep) \in ClassType))$;
%\item all other classes are $conc$.
%\end{itemize}
%
%Subject to minimizing the number of $dep$ classes, i.e.: 
%$$ minimize ~ \sum_{\forall c \in C} (c,dep) \in ClassType$$
%
%Having fixed the types of classes as above, we now have to solve a second optimization problem with restrictions R1 to R5.2 above to, having as inputs:
%\begin{itemize}
%\item the classes $C = \{c_1, .., c_{nc} \}$;
%\item $ClassConflict = C \times C$, the class conflict relation;
%\item $ClassType = C \times  \{ conc, dep\}$, where $conc$ means internally concurrent and $dep$ means internally dependent;
%\item $T = \{ t_1, .., t_{nt} \}$, the set of threads to map classes.
%\end{itemize}
%
%Our output should be 
%\begin{itemize}
%\item $CtoT = C \rightarrow \mathcal{P}(T)$.
%\end{itemize}
%
%To formulate the objective function for this second optimization step we adapt the concept of makespan \cite{????}  to our problem.
%\begin{itemize}
%\item Each thread of the system will be associated to $0$ to $nc$ classes.
%\item We compute the amount of work of each of the $nt$ threads when one unit of work for each
%of the $nc$ classes is submitted to the system.   We call the makespan of threat $t$ caused
%by class $c$, $ms_{(t,c)}$. The total makespan of threat $t$ due to all classes we call $ms_t$.  
%\item If a class $c_a$ is $conc$, associated to a subset of threads $T_a$, the
%the amount of work of each thread of this subset to accomplish a unit of work from $c_a$
%is assumed $1/card(T_a)$, which is $ms_{(i,c_a)}$.  $ms_{(i,c_a)}$ is added to $ms_i$ for all threads $i$ in $T_a$.
%\item If a class $c_b$ is internally conflicting, associated to a subset of threads $T_b$, the amount
%of work of each thread of this subset to accomplish a unit of work from $c_b$, $ms_{(j,c_b)}$, is assumed $1$,
%which is added to $ms_j$ for all threads $j$ in $T_b$.
%\item The objective function is to minimize the maximum makespan among all threads in the system.  
%\begin{itemize}
%\item This leads to a fair load distribution since minimizing the maximum will flatten the makespan value
%distribution across threads.  
%\item To minimize the maximum makespan also leads to minimizing the number of 
%overlapps among thread sets of different classes.  
%\item For independent classes, this leads to maximum thread usage, favoring concurrency.
%\end{itemize}


==> optimizer_copy.tex <==
%!TEX root =  main.tex
\section{Optimized scheduling in parallel \\ state machine replication}
\label{sec:optm}
\label{sec:optimization}

In this section, we formulate the problem of mapping a request classes definition to a set of worker threads.
The mapping assumes the execution model described in the previous section.

\subsection{The optimization model}

The mapping of threads to classes is shaped as an optimization problem that starting with some input data  must produce an output that satisfies a set of constraints and optimizes for a number of conditions (see Algorithm~\ref{model}).

\subsubsection{Input and output}
The input elements to the problem are:
\begin{itemize}
\item The set of classes $C = \{c_1, .., c_{nc} \}$.
\item The set of worker threads $T = \{ t_1, .., t_{nt} \}$.
\item The conflict relation $\#$ among classes $\# = C \times C$.
\item $W = C \times  \mathbb{R}$, the relative weight of internally non conflicting classes.  The weight is used to represent the work imposed by one class relative to the others and is used to accordingly distribute additional threads to concurrent classes.
\end{itemize}




\begin{itemize}
%\item The inputs are the request classes definition and a set of threads available;
\item A set of restrictions on the classes to threads mapping ensures that the execution is correct w.r.t. ordering;
\item The optimization function maximizes the throughput of the classes with the available working threads; and
\item The output is the classes to threads mapping as well as the definition of which classes are 
considered internally conflicting for the sake of thread synchronization.
\end{itemize}



%\subsubsection{Outputs} 
The optimization of this model has as outputs the mapping from classes to threads and the choice of which classes are considered internally conflicting according to discussed in IR.3 above.

\subsection{Constraints} 
%{\bf We then argue that the execution of this scheduling respects $\prec_R$ ?}.  

The set of restrictions to the mapping should ensure that implementation rules IR.0, IR.3, IR.4 and IR.5 are followed,
while IR.1 and IR.2 are ensured by the scheduler implementation.

\subsection{Objective function} 

The restrictions imposed by the implementation rules may be satisfied by several associations of threads to classes. 
Among those, we are interested in the ones where:
\begin{itemize}
\item O.1: internally concurrent classes use several threads to favor throughput;
\item O.2: thread distribution across concurrent classes consider the weight of the classes;
\item O.3: non conflicting classes with internal conflict use separate subsets of threads to avoid synchronization.
\end{itemize}




%The above discussed optimization model was implemented with AMPL \cite{AMPL} modeling language.


\begin{algorithm}[ht!]
\floatname{OptModel}{Model}
\caption{Optimization model.}
\footnotesize{
\begin{distribalgo}[1]
\label{model} 

\INDENT{\textbf{input:}}
%	\REQUIRE  \COMMENT{classes, conflicts and threads} \\
	\vspace{1mm}
	\STATE $set \ C$ \label{lC} 
	\COMMENT{\hfill // set of request classes}
	\vspace{1mm}
	\STATE $set \ T$ \label{lT}
	\COMMENT{\hfill // set of threads}
	\vspace{1mm}
	\STATE $w\{C\} \in [0..1]$ \label{lw}
	\COMMENT{\hfill // relative weight of each class}
	\vspace{1mm}
	\STATE $\#\{C_i,C_j\} \in \{ 0, 1 \}$ \label{lconflicts}
	\COMMENT{\hfill // $\#[c_i,c_j] = 1$\ :\ $c_i$ and $c_j$ conflict}
	\vspace{1mm}
%	\STATE $wc = \sum_{\forall c \in C\ :\ Cnc[c]} w[c]$
%	\COMMENT{\hfill // weights of concurrent classes}
%	\vspace{1mm}
\ENDINDENT

\INDENT{\textbf{output:}}
%	\REQUIRE \COMMENT{the mapping and internal conflict as in R2 } \\
	\vspace{1mm}
	\STATE $uses\{C,T\} \in \{ 0, 1 \}$ \label{luses} 
	\COMMENT{\hfill // uses[c,t] = 1 : class $c$ uses thread $t$}   
	\vspace{1mm}
	\STATE $Seq\{C\} \in \{ 0, 1 \}$ \label{ldep}
	\COMMENT{\hfill  // $Seq(c) = 1$ : $c$ is sequential}
	\vspace{1mm}
%	\STATE $Cnc\{C\} = \lnot Seq\{C\} \in \{ 0, 1 \}$ \label{ldep2}
%	\COMMENT{\hfill  // $Cnc(c) = 1$ : $c$ is concurrent}
%	\vspace{1mm}
\ENDINDENT

\INDENT{\textbf{auxiliary definitions:}}
	\vspace{1mm}
	\STATE $nc = |C|$
	\COMMENT{\hfill  // number of classes}
	
	\vspace{1mm}
	\STATE $nt = |T|$
	\COMMENT{\hfill  // number of worker threads}
	
	\vspace{1mm}
	\STATE $Cnc\{C\} = \lnot Seq\{C\} \in \{ 0, 1 \}$ \label{ldep2}
	\COMMENT{\hfill  // $Cnc(c) = 1$ : $c$ is concurrent}

	\vspace{1mm}
	\STATE $wc = \sum_{\forall c \in C\ :\ Cnc[c]} w[c]$
	\COMMENT{\hfill // weights of concurrent classes}

	\vspace{1mm}
\ENDINDENT


\INDENT{\textbf{constraints:}}
	\vspace{1mm}
	\STATE $\forall c \in C \ :\  \bigvee_{\forall t \in T} uses(c,t)$ \label{lIR0}
	\COMMENT{\hfill // R.0}
	\vspace{2mm}
	
	\STATE $\forall c \in C \ :\  \#[c_1,c_1] \Rightarrow Seq[c_1]$ \label{lIR1}
	\COMMENT{\hfill // R.1}
	\vspace{2mm}
	
	\STATE $\forall c_1, c_2 \in C \ :\ \#[c_1,c_2] \Rightarrow Seq[c_1] \lor Seq[c_2]$ \label{lIR3}
	\COMMENT{\hfill // R.3}
	\vspace{2mm}

	\STATE $\forall c_1, c_2 \in C, t \in T \ :\ $ \\
		\hfill $\#[c_1,c_2] \land Seq[c_1] \land Cnc[c_2] \land uses[c_2,t] \Rightarrow uses[c_1,t]$ \label{lIR4}
 	\COMMENT{\hfill // R.4}
	\vspace{2mm}

	\STATE $\forall c_1, c_2 \in C \ :\ \#[c_1,c_2] \land Seq[c_1] \land Seq[c_2] \Rightarrow $ \\
		\hfill $\exists t \in T \ :\ uses[c_1,t] \land uses[c_2,t]$ \label{lIR5}
	\COMMENT{\hfill // R.5}
	\vspace{1mm}
\ENDINDENT

 
\INDENT{\textbf{objective:}}
	\vspace{1mm}
	\STATE minimize cost:
	\vspace{2mm}

	\STATE $ - \sum_{\forall c \in C \,:\, Cnc[c]} |\{t \in T \,:\, uses[c,t]\}|$ \label{lobjinit}
	\COMMENT{\hfill // O.1}
	\vspace{2mm}

	\STATE $ + \sum_{\forall c \in C \,:\, Cnc[c]} w[c]/wc -$ \\
		\hfill $(|\{\forall t \in T:uses[c,t]\}|/ \mathit{nt} ) | \times \mathit{nt}$ \label{lobjloadb} 
	\COMMENT{\hfill // O.2}
	\vspace{2mm}

	\STATE $ + \sum_{\forall c_1, c_2 \in C \ s.t. \ Seq[c_1] \land Seq[c_2] \land \lnot \#[c_1,c_2]}$ \\
		\hfill $card(\{\forall t \in T \ s.t. \ uses[c_1,t] \land uses[c_2,t] \} )$ $\times 2 \times nt \times nc$ \label{lobjend} \label{lobj2ndpart}
	\COMMENT{\hfill // O.3}
	\vspace{2mm}
\ENDINDENT
      
\end{distribalgo}
}
\end{algorithm}

In lines \ref{lC} to \ref{lconflicts} we have the inputs to the problem, with the set of classes, their conflict relation, their relative weight and the set of threads to be mapped to.
As output we have the information if a given thread is used by a class, in line \ref{luses} and if the class is considered as internally sequential or concurrent for execution, see lines \ref{ldep} and \ref{ldep2}.
The restrictions discussed before are presented in lines \ref{lIR0} to \ref{lIR5}.  
In line \ref{lIR0} it is stated that for each class, at least one thread is associated.
In line \ref{lIR3} it is stated that if any two classes conflict then at least one of them is sequential.
In line \ref{lIR4} it is stated that if any two classes conflict, one of them is internally concurrent and the other sequential,
then all threads associated to the concurrent class are also in the sequential.
In line \ref{lIR5} it is stated that if any two classes conflict and both are sequential,
then there exists at least one common thread in both classes.

The objective function to minimize is presented in lines \ref{lobjinit} to \ref{lobjend}.
Beginning in \ref{lobjinit}, O.1, we have
a reward to the use of threads by internally concurrent classes, improving concurrency.
%
In O.2. we have that the use of threads by concurrent classes is proportional to their weight.  More concretely, we minimize the difference of the normalized weight of each class to its proportional use of available threads.  
We multiply this term by the number of threads in the system to make it compatible with the previous term.
%
The third part of the optimization function, O.3, applies a penalty to solutions that introduce common threads to non conflicting classes that have internal conflict.  The reason is that this would impose unneeded synchronization and thus impact throughput.
In line \ref{lobjend} we multiply this term such that it gains in priority with regard to the others.

%\subsection{Solving the optimization problem}
The optimization problem was described with the AMPL language \cite{fourer1993ampl} and solved with the KNitro solver \cite{Byrd06knitro:an}.

\subsection{Example}

Let us consider the generalized sharded service with single- and multi-shard read and write requests.
We take the example with 2 partitions, 8 threads, where all classes have same weight.  The input 
parameters are: set $C=\{C_{R1}, C_{W1}, C_{R2}, C_{W2}, C_{Rg}, C_{Wg} \}; set $T = \{1, 2, 3, 4, 5, 6, 7, 8\};
$w$, that associates 1 to all classes; and the conflict topology presented in Fig. \ref{fig:cclasses}(c) 
which is input in the $conflicts\{C,C\}$ parameter.

According to the optimization model, we have the following output to variable $Seq$:

 \begin{figure}[!ht]
  \begin{center}
  \includegraphics[width=0.9\columnwidth]{figs/classthreads1.pdf}
  \includegraphics[width=0.9\columnwidth]{figs/classthreads1.pdf}
  \end{center}
  \caption{Bla bla bla}
  \label{fig:classthreads}
\end{figure}



%%\begin{table}
%\begin{center}
%\begin{footnotesize}
%\begin{tabular}{|c|c|c|c|c|c|c|c|}
%\hline
%class    & $C_{Rg}$ & $C_{Wg}$ & $C_{R1}$  & $C_{R2}$ & $C_{W1}$ & $C_{W2}$  \\ 
%\hline
%Seq & T & T & F & F & T & T   \\ 
%\hline
%\end{tabular}
%\end{footnotesize}
%\end{center}
%% \caption{Output var $Sec\{C\}$}
%%\end{table} 
%
%The following thread association to each class in $uses$:
%
%\begin{center}
%\begin{footnotesize}
%\begin{tabular}{|c|c|c|c|c|c|c|c|}
%\hline
%& $C_{Rg}$ & $C_{Wg}$ & $C_{R1}$  & $C_{R2}$ & $C_{W1}$ & $C_{W2}$   \\ 
%\hline
%1 &  0 &  1 &  1  & 0  & 1 &  0  \\ \hline
%2 &  0 &  1 &  1  & 0  & 1 &  0 \\ \hline
%3 &  0 &  1 &  1  & 0  & 1 &  0 \\ \hline
%4 &  0 &  1 &  0  & 1  & 0 &  1 \\ \hline
%5 &  1 &  1 &  0  & 1  & 0 &  1 \\ \hline
%6 &  0 &  1 &  1  & 0  & 1 &  0 \\ \hline
%7 &  1 &  1 &  1  & 0  & 1 &  0 \\ \hline
%8 &  0 &  1 &  0  & 1  & 0 &  1 \\ \hline
%
%\end{tabular}
%\end{footnotesize}
%\end{center}
%% \caption{Output var $uses\{C,C\}$}
 
 
We notice that reads and writes in shards 1 and 2 use disjoint sets of threads, and that threads are distributed evenly among these classes.   Since reads in one shard can be concurrent but conflict with writes, the write class has all threads associated to the respective read class.   Global writes have to have a fixed order relative to all other operations, therefore all threads synchronize to execute a global write.    A global read is concurrent by the input conflict definition. Since $C_{Rg}$ conflicts with $C_{W1}$ and $C_{W2}$, to keep $C_{Rg}$ concurrent all threads that implement $C_{Rg}$ would have to be included in  $C_{W1}$ and $C_{W2}$.   Doing so, $C_{W1}$ and $C_{W2}$ would not be disjoint and thus synchronize even if no global read request is being processed.   A cheaper solution is to define $C_{Rg}$ as $Seq$ and associate to it one thread of each of the shards.  This means that whenever a global read takes place, it synchronizes its threads to execute in the shards.  Since writes in the shards are sequential, the global read will take place in a well defined order.
 
 


%
%
% while $c_2$ has no internal conflict, then the set of threads associated to $c_2$ must be included in the set of threads associated to $c1$.   This ensures that any request processed by $c_2$ has an order relative to $c_1$ because $c_1$ synchronize all its threads (which include those of $c_2$) to execute its requests. 
%
%\item R2: a thread may be associated to any number of classes, from 0 to $nc$; 
%\item R3: a class without internal conflict $c_c$ ($c$oncurrent) schedules a request to any one of its threads;
%\item R4: a class with internal conflict $c_d$ ($d$ependent) schedules a request to all of its threads (see execution model);
%
%\item R5: different, conflicting classes have to have overlapping sets of threads;
%\item R5.1: if two internally conflicting classes conflict, then they need at least one common thread to assure total order among them (see R4);
%\item R5.2: if one internally conflicting class $c_d$ conflicts with one internally non-conflicting class $c_c$, it suffices that threads of $c_c$ are contained in threads of $c_d$.  Since $c_d$ schedules the requests to all its threads, the synchronous execution of a request in all of $c_c$ threads creates a  total order among classes, although $c_c$ requests are concurrent among them;
%\item R5.3: if two internally non conflicting classes conflict (even this case may be rare), the total order among classes has to be respected.   It suffices to reduce this case to R5.2 by assuming as if one of the classes would be internally conflicting and thus granting the same as R5.2.
%\end{itemize}
%
%The choice of which classes should be considered internally conflicting (discussed R5.3) should minimize the number of 
%internally conflicting classes in the system, since they reduce concurrency. This choice depends only on the topology of dependencies among classes and is irrespective of the mapping to threads.  
%We solve this problem in a separate optimization problem, before mapping threads to classes, defined as follows.

%Given inputs:
%\begin{itemize}
%\item the classes $C = \{c_1, .., c_{nc} \}$;
%\item $ClassConflict = C \times C$, the class conflict relation;
%\end{itemize}
%
%Calculate the output:
%\begin{itemize}
%\item $ClassType = C \times  \{ conc, dep\}$, where $conc$ means internally concurrent and $dep$ means internally dependent;
%\end{itemize}
%
%With the following restrictions:
%\begin{itemize}
%\item if a class conflicts internally, it is of type $dep$, i.e.:  $\forall (c,c) \in ClassConflict, (c,dep) \in ClassType$;
%\item if two classes conflict, at least one is $dep$, i.e.: $\forall (c_a, c_b) \in ClassConflict, ((c_a,dep) \in ClassType) \vee (c_b,dep) \in ClassType))$;
%\item all other classes are $conc$.
%\end{itemize}
%
%Subject to minimizing the number of $dep$ classes, i.e.: 
%$$ minimize ~ \sum_{\forall c \in C} (c,dep) \in ClassType$$
%
%Having fixed the types of classes as above, we now have to solve a second optimization problem with restrictions R1 to R5.2 above to, having as inputs:
%\begin{itemize}
%\item the classes $C = \{c_1, .., c_{nc} \}$;
%\item $ClassConflict = C \times C$, the class conflict relation;
%\item $ClassType = C \times  \{ conc, dep\}$, where $conc$ means internally concurrent and $dep$ means internally dependent;
%\item $T = \{ t_1, .., t_{nt} \}$, the set of threads to map classes.
%\end{itemize}
%
%Our output should be 
%\begin{itemize}
%\item $CtoT = C \rightarrow \mathcal{P}(T)$.
%\end{itemize}
%
%To formulate the objective function for this second optimization step we adapt the concept of makespan \cite{????}  to our problem.
%\begin{itemize}
%\item Each thread of the system will be associated to $0$ to $nc$ classes.
%\item We compute the amount of work of each of the $nt$ threads when one unit of work for each
%of the $nc$ classes is submitted to the system.   We call the makespan of threat $t$ caused
%by class $c$, $ms_{(t,c)}$. The total makespan of threat $t$ due to all classes we call $ms_t$.  
%\item If a class $c_a$ is $conc$, associated to a subset of threads $T_a$, the
%the amount of work of each thread of this subset to accomplish a unit of work from $c_a$
%is assumed $1/card(T_a)$, which is $ms_{(i,c_a)}$.  $ms_{(i,c_a)}$ is added to $ms_i$ for all threads $i$ in $T_a$.
%\item If a class $c_b$ is internally conflicting, associated to a subset of threads $T_b$, the amount
%of work of each thread of this subset to accomplish a unit of work from $c_b$, $ms_{(j,c_b)}$, is assumed $1$,
%which is added to $ms_j$ for all threads $j$ in $T_b$.
%\item The objective function is to minimize the maximum makespan among all threads in the system.  
%\begin{itemize}
%\item This leads to a fair load distribution since minimizing the maximum will flatten the makespan value
%distribution across threads.  
%\item To minimize the maximum makespan also leads to minimizing the number of 
%overlapps among thread sets of different classes.  
%\item For independent classes, this leads to maximum thread usage, favoring concurrency.
%\end{itemize}


==> whyitworksDiferentConfigs.tex <==

\subsubsection{Why it works}   
\label{sec.whyitworksDifferentConfigs}

%Here we argue that replicas with different numbers of working threads generate the same results, i.e., their runs are executions of $\prec_R$.
The general argument is that Proposition \ref{prop.CorrectReplicaRun} is independent of the number of threads.
%The general argumentation is that if each replica respects $\prec_R$, then their executions generate the same results.
%
In more detail, Algorithms \ref{alg_scheduler_dc} and \ref{alg_workers_dc} 
only differ from Algorithms \ref{alg_scheduler} and \ref{alg_workers}, respectively, in that they verify if the set of conflicting threads returned by function $CtoT$ is supported by the replica's configuration. 
If it is, Algorithms \ref{alg_scheduler_dc} and \ref{alg_workers_dc} behave as Algorithms \ref{alg_scheduler} and \ref{alg_workers}.
Otherwise, Algorithms \ref{alg_scheduler_dc} and \ref{alg_workers_dc} synchronize all threads to execute the request.   
This preserves safety since this enforces the total delivery order in such cases, which is always correct.
All executions will preserve the total order of conflicting requests, which satisfies $\prec_R$.








==> whyitworksReconfigurable.tex <==

\subsubsection{Why it works}   

%Here we argue that the above described execution model respects $\prec_R$ as discussed in Section \ref{sec:paralellismInSMR}, even having replicas reconfiguring on-the-fly their parallelism level.

To keep the execution safe it has to be shown that the replica run satisfies $\prec_R$ even if the replica is reconfigured to a different number of working threads.
As already argued in Section \ref{sec.whyitworksDifferentConfigs}, replicas with different number of threads subject to the same request sequence $(R,<_R)$ generate the same results (satisfy $\prec_R$). Since the number of threads is not important to keep safety, correctly switching the number of active threads will generate safe executions.
%varying the number of threads while keeping the execution safe will generate the same results.  
We substantiate this claim by showing that the computation before and after the reconfiguration is generated correctly.   

%The scheduler is sequential, i.e. append operations to all thread queues are sequential. 
When the scheduler decides to change the number of threads (i.e., update $n'$), 
a $reconfig(n')$ request is appended to all ($maxThreads$) threads.  At this moment it is the last request of all queues
and all threads synchronize to execute it.   With this we have a point of reference in the concurrent execution of worker threads.
%
Now we argue that requests before this point of reference are processed correctly.
Any request processed before $reconfig$ is enqueued is assumed correct by previous argumentation (algorithms without reconfiguration)
since the logic is the same.
Any request prior to an enqueued $reconfig$ was enqueued considers the previous value of $n$.
Since the barrier $bAll$ is only modified when $reconfig$ is executed (and not when it is enqueued),
$bAll$ accords to the value of $n$ previous to reconfiguration and thus involves the correct number of active threads
before $reconfig$.   By previous argumentation, the prefix before $reconfig$ is correct. 

Now we argue about the correct processing after $reconfig$.
$reconfig$ is executed in mutual exclusion.
It changes the value of $bAll$ and $n$ according to the new number of threads informed in the request $reconfig(n')$.
According to the scheduler, any request enqueued after $reconfig$ 
considered the new number of active threads $n'$.
When $reconfig$ takes place it updates $bAll$ and $n$ (which is used in worker threads) 
to the new value $n'$.   Therefore after the point of reference provided by $reconfig$, the number of
active threads considered $n$ accord to the barrier $bAll$ and to $n'$ (i.e., the number of active threads
considered by the scheduler after the respective $reconfig(n')$ was issued).  
%Thus, requests 
%after $config$ will be executed considering the correct number of active threads and with
%the correct configuration of the barrier.   
This establishes a correct execution after $reconfig$.   
Since $n'$ is only used at the scheduler and the new $n$ for worker threads is informed in the 
$reconfig(n')$ message, one can observe that several enqueued $reconfig$ messages with
different number of active threads are possible and the service requests enqueued between any two
$reconfigs$ are processed with the correct values of $n$ and $bAll$ at worker threads.
It is also clear that the $reconfig$ process does not lose, insert, or change the order
of requests in the queues.


%%::::: acho que o abaixo nao precisa mais \ct{Falta provar o item i ?}
%%
%%(ii) that a command execution starts and finishes in a same consistent replica configuration, and 
%%
%%(iii) that the reconfiguration procedure does not harm $\prec_C$ while it starts in a consistent replica configuration and leaves the replica configuration consistent.
%%
%%
%%
%%
%%
%%% -----------------------
%%
%%


==> whyitworksconcurrent.tex <==
%!TEX root =  rp_smr-v3.tex

\subsubsection{Why it works}   

Here we argue that the above described execution model respects $\prec_R$ as discussed in Section \ref{sec:paralellismInSMR}.

\begin{definition}[Replica]
\label{def.replica}
Given a request sequence  $(R,<_R)$, a \emph{replica}  $Rp$ is a finite set of worker threads that execute this request sequence, that is
 $Rp = \{ WT_i | 0 \leq i \leq n-1, n \in \mathbb{N}, WT_i = (R_i,<_{R_i}) \mbox{ is also a request sequence}\}$
such that (see Algorithm 1):

{\bf i)}  All requests in $R$ are enqueued at some worker thread: $ \bigcup_{0\leq i \leq n-1} R_i = R$; which
is granted since every delivered request is assigned either to one thread (no conflict case); 
or to a subset of conflicting threads.

{\bf ii)} The queues of the worker threads are compatible with the request sequence order: $<_{R_i} = <_R |_{R_i}$;
$<_R$ is represented by the total delivery order.
Since $on$ $deliver$ is performed in the delivery order, the scheduler appends requests to threads in the correct sequence.
The total order of each $<_{R_i}$ is compatible  with $<_{R}$.

%and worker threads process requests in sequence (l. 27), i.e. FIFO for each thread, the total order of $<_{B_i}$ compatible  with $<_{B}$.
{\bf iii)} A request is in multiple threads if and only if it depends on items on those threads:
         $r \in R_i \mbox{ and } r\in R_j \mbox{ with } i\neq j \Leftrightarrow
         (\exists r_i \in R_i, r_j\in R_j, r_i \prec_R r \mbox{ and } r_j \prec_R r)$. 
% 
This is ensured by $on$ $deliver$.  It identifies conflicts with all involved threads and enqueues the request to all of them.

Considering that each replica has the same conflict classes,
%\odo{definition, given by function $r\_map$,}
%definition (see Definition \ref{def.welldefReplica}), 
requests will be enqueued to the same threads and thus induce the same dependencies.
Note that since $<_{R_i}$ is an image of $<_R$, the dependency relation on requests of $R_i$, $\prec_{R_i}$, must be $\prec_R$ restricted to the items in $R_i$.
\end{definition}
 





\begin{definition}[Replica run]
\label{def.replicarun}
Given a $Rp$ with $n$ worker threads $WT$ over a request sequence  $(R,<_R)$, a  complete
\emph{run  $\pi$ of replica} $Rp$ is a list defined inductively as follows ($\bullet$ denotes the inclusion of an element in front of a list):
\begin{enumerate}
\item [i)] $\pi$ is the empty list if all worker threads are empty;

\item [ii)] $\pi = r \bullet \pi'$ if 
         
         {\bf a)} $r$ is the first request of a set of $m$ worker threads of $Rp$ and $r$ does not appear in any other worker thread.
         
         {\bf b)}
         $\pi'$ is the replica run of the replica $R'$ obtained by removing $r$ from all worker threads in which it appeared. 
         
         This behavior is implemented in Algorithm 2. In case $r$ appears in only one queue the thread executes it.
         Otherwise every involved worker thread eventually dequeues $r$ and enters a barrier with other threads in $classId$. 
         Only one thread executes $r$ and all other threads wait for it to complete.    
\end{enumerate}
\end{definition}

Given the formalization above of a replica run, now we have to discuss that such a run is an execution of  $\prec_R$ which has been argued to be linearizable.

 \begin{proposition}
 \label{prop.CorrectReplicaRun}
Replica run is an execution of $\prec_R$. 

Proof:
% well-defined (Liveness - it is always possible to obtain a replica run). Proof:
%\end{proposition}
%
%\begin{proof}
\emph{The run $\pi$ of a replica is:}
\begin{enumerate}
\item [i)] \emph{the empty list: the empty execution satisfies $\prec_R$;}

\item [ii)] \emph{$\pi = r \bullet \pi'$, in which case we have to show that the choice of executing $r$ respects $\prec_R$.}%$ divided in the following cases: 
%          \begin{description}
%          \item [a)]
%          $c$ is the first request of one thread $WT_i$ of $R$ and $c$ does not appear in any other working thread.   
%          In such case, according to Def. \ref{def.replica} either $c$ conflicted with requests of that single thread or was an independent request.
%          Each separate $\prec_{C_i}$ was already shown to be compatible with $\prec_R$.  
%          In the first case $c$ conflicts with requests in $C_i$ and is independent of any requests in $C_j, j\neq i$,
%          it has a correct order in $\prec_R_i$.
%          In the second case $c$ is an independent request and could assume any order in any $WT$, since it is assigned to a $WT_i$ which executes requests in FIFO, $c$ is eventually executed.
%          
%         \item [b)]
         \emph{ ~$r$ is the first request of a set of $m$ worker threads of $Rp$ and $r$ does not appear in any other worker thread.
          In this case $r$ conflicted with requests of threads in $m$, according to Def. \ref{def.replica}.iii.}
          %When $c$ is the first request of all threads in $m$, all dependencies in $\prec_R$ were solved and $c$ can execute.
          \emph{For each thread $WT_i$ in $m$, $r$ respects $\prec_{R_i}$, as discussed.  Since %all requests of 
          $\bigcup_{0\leq i \leq n-1} R_i = R$ (Def. \ref{def.replica}.i) and since a request $r$ is in multiple threads iff it depends in items on those threads (Def. \ref{def.replica}.iii), each dependency relation $\prec_{R_i}$ is compatible with $\prec_R$ and all dependencies of $r$ on other requests in $(R,\prec_R)$ are accordingly mapped to $\prec_{R_i} \in m$.
          This ensures that the execution $r \bullet \pi'$  respects $\prec_R$.
          The case where $r$ appears in a single thread is a particular case where $m$ has only one thread. Either $r$ conflicted with prior requests for the thread or $r$ is independent.   The first case is correct due to the Fifo execution.  In the second case, 
          independent requests are assigned to some $R_i$, having a valid order since any order would suffice.}
          
          
          
%         \item [b)] 
%         $\pi'$ is the replica run of the replica $R'$ obtained by removing $c$ from all working threads in which it appeared. 
%         
%         This behaviour is implemented in Algorithm 2. In case $c$ appears in only one queue the thread executes it (lines 3, 4).
%         Otherwise (lines 5 to 13) every involved worker thread eventually dequeues $c$ and executes it and enters a barrier with other threads in $groupId$. 
%         Only the thread executes $c$ (line 8) and all other threads wait for it to complete (lines 11, 12).    
%         %\end{description}
\end{enumerate}
\emph{Since a replica run is an execution of $\prec_R$, according to Proposition \ref{prop.safeExecution}  a replica run is safe.} $\strut\hfill \Box$
\end{proposition}














